DEPART: DEcomposing PARiTy across Multilingual LLMs

Multilingual Large Language Models (mLLMs) leaderboards report per-language accuracy but rarely explain why disparities emerge, leaving systemic biases unattributed and offering practitioners no actionable levers. We first establish that these gaps are systematic rather than artifacts of sampling noise via distribution-free Friedman and Kruskal--Wallis tests, then introduce a two-step Bayesian hierarchical framework that decomposes multilingual performance variance into interpretable components. First, isolating the variance attributable to language identity, we show that observable language features (script, family, typological distance) explain $R^2_{\text{ling}} = 79\%$ of this variance on understanding tasks and $92\%$ on reasoning, with a model's internal representational similarity to English emerging as the dominant predictor across both task buckets. Second, decomposing the full (model$\times$benchmark$\times$language) cube, we find that NLU and reasoning have fundamentally divergent variance profiles: model identity dominates understanding ($66.7\%$ of variance), whereas the benchmark$\times$model interaction dominates reasoning ($46.3\%$). Together these results recast multilingual evaluation from passive performance mapping into an explainable, diagnostic framework with concrete levers for targeting the root drivers of language disparity.

==> sections/01_introduction.tex <==
\section{Introduction}
\paragraph{Motivation} Large Language Models (LLMs) are deployed worldwide, yet their performance varies sharply across the languages they serve, producing systematically worse outputs for speakers of low-resource languages \citep{Choudhury_Deshpande_2021, khanuja-etal-2023-evaluating}.
The field measures this gap using per-language tables, occasional Gini coefficients, ``English vs.\ X'' deltas, but does not yet explain it.
% The substantive question that motivates this work is: \emph{what share of cross-language performance gaps is structurally predictable (from language and model representation features) versus model-specific?}
The substantive question that motivates this work is sharper than \emph{how big is the gap?}, we instead ask \emph{what fraction of the cross-language gap is predictable before any benchmark is run}, using observable language properties (script, family, typological distance, resource class) and cheap model-conditional probes (tokenizer fertility, internal representation similarity to English) and \emph{what fraction is an irreducible per-checkpoint residual}?

The answer determines where interventions could be most consequential: 
\textbf{\textit{(1)}} feature-predictable disparity points to data and 
tokenization choices made prior to training, whereas \textit{\textbf{(2)}} 
a large model-specific residual would indicate checkpoint-level idiosyncrasies 
that only retraining can address. To account for these model-specific details, 
such as architectural choices and training data composition (which is otherwise 
difficult to estimate due to the opaqueness of data releases), we selected these 
features and additionally incorporated model and benchmark-level effects as inputs.


% The answer determines where intervention could be most consequential: \textbf{\textit{(1)}} feature-predictable disparity points to data and \textit{\textbf{(2)}} tokenization choices made before training, while a large model-specific residual would point to checkpoint-level idiosyncrasies that only retraining can address. We chose these features, and in addition added model and task level effects as inputs to our model to account for model specific details, be it training data composition (which is hard to estimate otherwise given the opaqueness in data release) and architecural choices.

\paragraph{Research Gap} Existing work addresses this question partially: fairness frameworks \citep{Choudhury_Deshpande_2021, khanuja-etal-2023-evaluating} reduce disparity to one-dimensional statistics (Gini, max--min); the closest methodological precedent \citep{hu-etal-2025-quantifying} fits an additive mixed-effects model that ranks languages by difficulty but cannot identify model$\times$language interactions or incorporate linguistic covariates; similarity rankings \citep{Li_Shi_Liu_Yang_Payani_Liu_Du_2025} and proxy-LM forecasts \citep{anugraha-etal-2025-proxylm} contribute individual signals without a fairness-style decomposition (Section~\ref{sec:related}). To our knowledge, no prior work provides a unified hierarchical decomposition that jointly attributes observed disparity to structural and model-specific components, with calibrated uncertainty for both.

% Existing work approaches this question in pieces: normative fairness frameworks \citep{Choudhury_Deshpande_2021, khanuja-etal-2023-evaluating} operationalise disparity through one-dimensional summary statistics (Gini, max--min); the closest methodological precedent \citep{hu-etal-2025-quantifying} fits an additive mixed-effects model that ranks languages by difficulty but cannot, by construction, identify model$\times$language interactions or admit linguistic features as covariates; intrinsic-similarity rankings \citep{Li_Shi_Liu_Yang_Payani_Liu_Du_2025} and proxy-LM forecasts \citep{anugraha-etal-2025-proxylm} contribute individual signals without a fairness-style decomposition (see Section~\ref{sec:related}).
% What is missing is a single hierarchical decomposition that jointly attributes observed disparity to structural components (predictable from language- and model-level features) and a residual model-specific component, with calibrated uncertainty on both.

\begin{figure*}
    \centering \includegraphics[width=\textwidth,keepaspectratio]{latex/figures/title_figure_v3.pdf}
    \caption{Structural factors dominate cross-lingual performance gaps in multilingual LLMs.}
    \label{fig:main}
\end{figure*}

\paragraph{Approach} We evaluate 7 open-weight LLMs ($\sim$3.5B--122B parameters) on 15 multilingual benchmarks covering 63 languages, partitioned into \textbf{\textit{(1)}} multilingual-understanding (9 benchmarks, 63 languages) and \textbf{\textit{(2)}} reasoning (6 benchmarks, 62 languages) task buckets.
We fit a Bayesian hierarchical model that jointly estimates the contribution of the model, benchmark, language, interactions, and observable \textbf{\textit{(1)}} language-level and \textbf{\textit{(2)}} model$\times$language features --- resource class \citep{joshi-etal-2020-state}, lang2vec syntactic, phonological, and geographic distance to English \citep{littell-etal-2017-uriel}, script, family, tokenizer fertility, and the alignment between a model's representation of a language and its representation of English.
The following are the key contributions of this work:
\begin{enumerate}
    \item \textbf{Non-parametric validation of widespread language disparity.} Before applying structural decompositions, we deploy distribution-free statistical tests to verify that observed cross-lingual gaps are systematic rather than artifacts of sampling noise. A Friedman test rejects the null hypothesis of equal language ranks across all 18 benchmarks ($W$ up to $0.91$, median $\sim0.75$), while a Kruskal-Wallis omnibus followed by Dunn pairwise tests decisively rejects performance equality across Joshi resource tiers ($p < 10^{-15}$), proving that performance drops are rigidly structured by a language's resource level.
    % \item \textbf{A joint hierarchical decomposition of multilingual disparity.} We introduce $R^2_{\text{ling}}$, the proportional reduction in the language random-intercept variance attributable to observable features --- a principled, uncertainty-quantified answer to \emph{how much of the cross-language gap is structural} that prior additive specifications cannot deliver.
    % \item \textbf{Quantification of the gap and its structural share.} Holding model and benchmark fixed, languages deviate by $\pm 8$--$9$ accuracy points on average ($\sigma_\alpha = 0.078$ on understanding, $0.088$ on reasoning); observable language features alone recover $R^2_{\text{ling}} = 0.79$ on understanding and $0.92$ on reasoning ($90\%$ HDIs $[0.57, 0.93]$ and $[0.73, 0.99]$), showing that most of the cross-language variation is predictable from properties known in advance of evaluation. Across both task buckets, a model's internal representation alignment to English emerges as the single most dominant predictor: a one-SD increase is worth $+6.5$ accuracy points on understanding and $+9.4$ on reasoning, offering a benchmark-free proxy computable from the model geometry alone
    \item \textbf{A joint hierarchical decomposition of multilingual disparity.} We fit a Bayesian hierarchical model that estimates how much of the cross-language gap is explained by observable features and how much remains as an irreducible residual, with calibrated uncertainty on each component. We summarise the explanatory share by $R^2_{\text{ling}}$, defined as the proportional reduction in the language random-intercept variance once observable features are added --- a principled, uncertainty-quantified answer to \emph{how much of the cross-language gap is predictable in advance} that prior additive specifications cannot deliver.
    \item \textbf{Quantification of the gap and its predictable share.} Holding model and benchmark fixed, languages deviate by $\pm 8$--$9$ accuracy points on average --- the cross-language standard deviation $\sigma_\alpha = 0.078$ on understanding and $0.088$ on reasoning, where $\sigma_\alpha$ is the posterior SD of the language random intercept. Observable language features alone recover $R^2_{\text{ling}} = 0.79$ on understanding and $0.92$ on reasoning ($90\%$ HDIs $[0.57, 0.93]$ and $[0.73, 0.99]$), showing that most of the cross-language variation is predictable from properties measurable in advance of evaluation. Across both task buckets, a model's internal representation alignment to English emerges as the single most dominant predictor: a one-SD increase is worth $+6.5$ accuracy points on understanding and $+9.4$ on reasoning, offering a benchmark-free proxy computable from the model geometry alone.
    \item \textbf{A clear decomposition of the variance causing elements} Model identity dominates understanding ($66.7\%$ of total variance), whereas benchmark$\times$model interaction dominates reasoning ($46.3\%$, larger than the main model effect), so a single ``multilingual reasoning'' aggregate is misleading and per-benchmark reporting is warranted.
\end{enumerate}


==> sections/dunns_table.tex <==
% ============================================================
%  Dunn's post-hoc on Joshi resource classes
%  BH-corrected pairwise p-values. *** p<.001, ** p<.01, * p<.05, ns p>=.05.
%  Class labels (Joshi et al., 2020): 1=Scraping, 2=Hopefuls, 3=Rising,
%  4=Underdogs, 5=Winners.  All p-values are symmetric; matrices show full grid
%  for readability.  Source: scikit_posthocs.posthoc_dunn(..., p_adjust="fdr_bh")
%  on within-(model, benchmark) z-scored per-language scores.
% ============================================================

% Reusable compact column type
\newcommand{\dcell}[1]{\multicolumn{1}{c}{#1}}


\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l ccccc}
\toprule
 & 1 & 2 & 3 & 4 & 5 \\
\midrule
1 & ---                 & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,*** \\
2 & $<\!10^{-4}$\,***   & ---                & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,*** \\
3 & $<\!10^{-4}$\,***   & $<\!10^{-4}$\,***  & ---                & .0886\,ns          & $<\!10^{-4}$\,*** \\
4 & $<\!10^{-4}$\,***   & $<\!10^{-4}$\,***  & .0886\,ns          & ---                & .0001\,*** \\
5 & $<\!10^{-4}$\,***   & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & .0001\,***         & --- \\
\bottomrule
\end{tabular}
\caption{Qwen3.5-122B-A10B, NLU.}
\label{tab:dunn_qwen122b_nlu}
\end{table*}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l ccccc}
\toprule
 & 1 & 2 & 3 & 4 & 5 \\
\midrule
1 & ---           & .0311\,*           & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,*** \\
2 & .0311\,*      & ---                & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,*** \\
3 & $<\!10^{-4}$\,*** & $<\!10^{-4}$\,*** & ---            & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,*** \\
4 & $<\!10^{-4}$\,*** & $<\!10^{-4}$\,*** & $<\!10^{-4}$\,*** & ---             & .0021\,** \\
5 & $<\!10^{-4}$\,*** & $<\!10^{-4}$\,*** & $<\!10^{-4}$\,*** & .0021\,**       & --- \\
\bottomrule
\end{tabular}
\caption{Qwen3.5-4B, NLU.}
\label{tab:dunn_qwen4b_nlu}
\end{table*}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l ccccc}
\toprule
 & 1 & 2 & 3 & 4 & 5 \\
\midrule
1 & ---                 & .0003\,***         & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,*** \\
2 & .0003\,***          & ---                & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,*** \\
3 & $<\!10^{-4}$\,***   & $<\!10^{-4}$\,***  & ---                & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,*** \\
4 & $<\!10^{-4}$\,***   & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & ---                & .0328\,* \\
5 & $<\!10^{-4}$\,***   & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & .0328\,*           & --- \\
\bottomrule
\end{tabular}
\caption{aya-expanse-32b, NLU.}
\label{tab:dunn_aya32b_nlu}
\end{table*}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l ccccc}
\toprule
 & 1 & 2 & 3 & 4 & 5 \\
\midrule
1 & ---                & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,*** \\
2 & $<\!10^{-4}$\,***  & ---                & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,*** \\
3 & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & ---                & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,*** \\
4 & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & ---                & .0011\,** \\
5 & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & .0011\,**          & --- \\
\bottomrule
\end{tabular}
\caption{gpt-oss-20b, NLU.}
\label{tab:dunn_gptoss_nlu}
\end{table*}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l ccccc}
\toprule
 & 1 & 2 & 3 & 4 & 5 \\
\midrule
1 & ---                & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,*** \\
2 & $<\!10^{-4}$\,***  & ---                & .5950\,ns          & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,*** \\
3 & $<\!10^{-4}$\,***  & .5950\,ns          & ---                & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,*** \\
4 & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & ---                & $<\!10^{-4}$\,*** \\
5 & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & --- \\
\bottomrule
\end{tabular}
\caption{sarvam-105b, NLU.}
\label{tab:dunn_sarvam105_nlu}
\end{table*}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l ccccc}
\toprule
 & 1 & 2 & 3 & 4 & 5 \\
\midrule
1 & ---                & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,*** \\
2 & $<\!10^{-4}$\,***  & ---                & .3295\,ns          & .4224\,ns          & $<\!10^{-4}$\,*** \\
3 & $<\!10^{-4}$\,***  & .3295\,ns          & ---                & .6598\,ns          & $<\!10^{-4}$\,*** \\
4 & $<\!10^{-4}$\,***  & .4224\,ns          & .6598\,ns          & ---                & $<\!10^{-4}$\,*** \\
5 & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & --- \\
\bottomrule
\end{tabular}
\caption{sarvam-30b, NLU.}
\label{tab:dunn_sarvam30_nlu}
\end{table*}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l ccccc}
\toprule
 & 1 & 2 & 3 & 4 & 5 \\
\midrule
1 & ---                & .0862\,ns          & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,*** \\
2 & .0862\,ns          & ---                & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,*** \\
3 & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & ---                & $<\!10^{-4}$\,***  & .0001\,*** \\
4 & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & ---                & .0830\,ns \\
5 & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & .0001\,***         & .0830\,ns          & --- \\
\bottomrule
\end{tabular}
\caption{tiny-aya-global, NLU.}
\label{tab:dunn_tinyaya_nlu}
\end{table*}


% ---------- PER-MODEL REASONING ----------

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l ccccc}
\toprule
 & 1 & 2 & 3 & 4 & 5 \\
\midrule
1 & ---         & .8552\,ns          & .0142\,*           & .0105\,*           & .0260\,* \\
2 & .8552\,ns   & ---                & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & .0105\,* \\
3 & .0142\,*    & $<\!10^{-4}$\,***  & ---                & .8007\,ns          & .8007\,ns \\
4 & .0105\,*    & $<\!10^{-4}$\,***  & .8007\,ns          & ---                & .8007\,ns \\
5 & .0260\,*    & .0105\,*           & .8007\,ns          & .8007\,ns          & --- \\
\bottomrule
\end{tabular}
\caption{Qwen3.5-122B-A10B, Reasoning.}
\label{tab:dunn_qwen122b_reasoning}
\end{table*}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l ccccc}
\toprule
 & 1 & 2 & 3 & 4 & 5 \\
\midrule
1 & ---           & .9191\,ns          & .0210\,*           & .0010\,***         & .0010\,*** \\
2 & .9191\,ns     & ---                & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,*** \\
3 & .0210\,*      & $<\!10^{-4}$\,***  & ---                & .0408\,*           & .0394\,* \\
4 & .0010\,***    & $<\!10^{-4}$\,***  & .0408\,*           & ---                & .2596\,ns \\
5 & .0010\,***    & $<\!10^{-4}$\,***  & .0394\,*           & .2596\,ns          & --- \\
\bottomrule
\end{tabular}
\caption{Qwen3.5-4B, Reasoning.}
\label{tab:dunn_qwen4b_reasoning}
\end{table*}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l ccccc}
\toprule
 & 1 & 2 & 3 & 4 & 5 \\
\midrule
1 & ---           & .5501\,ns          & .0464\,*           & .0015\,**          & .0002\,*** \\
2 & .5501\,ns     & ---                & .0088\,**          & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,*** \\
3 & .0464\,*      & .0088\,**          & ---                & .0071\,**          & .0016\,** \\
4 & .0015\,**     & $<\!10^{-4}$\,***  & .0071\,**          & ---                & .0500\,ns \\
5 & .0002\,***    & $<\!10^{-4}$\,***  & .0016\,**          & .0500\,ns          & --- \\
\bottomrule
\end{tabular}
\caption{aya-expanse-32b, Reasoning.}
\label{tab:dunn_aya32b_reasoning}
\end{table*}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l ccccc}
\toprule
 & 1 & 2 & 3 & 4 & 5 \\
\midrule
1 & ---         & .0755\,ns   & .9072\,ns   & .2782\,ns   & .0240\,* \\
2 & .0755\,ns   & ---         & .0004\,***  & .1282\,ns   & .2250\,ns \\
3 & .9072\,ns   & .0004\,***  & ---         & .0240\,*    & .0018\,** \\
4 & .2782\,ns   & .1282\,ns   & .0240\,*    & ---         & .0431\,* \\
5 & .0240\,*    & .2250\,ns   & .0018\,**   & .0431\,*    & --- \\
\bottomrule
\end{tabular}
\caption{gpt-oss-20b, Reasoning.}
\label{tab:dunn_gptoss_reasoning}
\end{table*}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l ccccc}
\toprule
 & 1 & 2 & 3 & 4 & 5 \\
\midrule
1 & ---         & .1318\,ns   & .8575\,ns   & .1318\,ns   & .0268\,* \\
2 & .1318\,ns   & ---         & .0073\,**   & .8575\,ns   & .1562\,ns \\
3 & .8575\,ns   & .0073\,**   & ---         & .0063\,**   & .0063\,** \\
4 & .1318\,ns   & .8575\,ns   & .0063\,**   & ---         & .1318\,ns \\
5 & .0268\,*    & .1562\,ns   & .0063\,**   & .1318\,ns   & --- \\
\bottomrule
\end{tabular}
\caption{sarvam-105b, Reasoning.}
\label{tab:dunn_sarvam105_reasoning}
\end{table*}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l ccccc}
\toprule
 & 1 & 2 & 3 & 4 & 5 \\
\midrule
1 & ---         & .0349\,*   & .4451\,ns  & .1495\,ns  & .1325\,ns \\
2 & .0349\,*    & ---        & .0027\,**  & .1053\,ns  & .8418\,ns \\
3 & .4451\,ns   & .0027\,**  & ---        & .1495\,ns  & .1495\,ns \\
4 & .1495\,ns   & .1053\,ns  & .1495\,ns  & ---        & .4253\,ns \\
5 & .1325\,ns   & .8418\,ns  & .1495\,ns  & .4253\,ns  & --- \\
\bottomrule
\end{tabular}
\caption{sarvam-30b, Reasoning.}
\label{tab:dunn_sarvam30_reasoning}
\end{table*}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l ccccc}
\toprule
 & 1 & 2 & 3 & 4 & 5 \\
\midrule
1 & ---           & .6452\,ns          & .0209\,*           & .0015\,**          & .0002\,*** \\
2 & .6452\,ns     & ---                & .0006\,***         & $<\!10^{-4}$\,***  & $<\!10^{-4}$\,*** \\
3 & .0209\,*      & .0006\,***         & ---                & .0531\,ns          & .0044\,** \\
4 & .0015\,**     & $<\!10^{-4}$\,***  & .0531\,ns          & ---                & .0488\,* \\
5 & .0002\,***    & $<\!10^{-4}$\,***  & .0044\,**          & .0488\,*           & --- \\
\bottomrule
\end{tabular}
\caption{tiny-aya-global, Reasoning.}
\label{tab:dunn_tinyaya_reasoning}
\end{table*}

==> tables/tree_tables.tex <==
\input{tables/tree_holdout.tex}
\input{tables/tree_holdout_joshi.tex}
\input{tables/tree_importance.tex}


